Version Age of Information Minimization over Fading Broadcast Channels

We consider a base station (BS) that receives version update packets from multiple exogenous streams and broadcasts them to corresponding users over a fading broadcast channel using a non-orthogonal multiple access (NOMA) scheme. Sequentially indexed packets arrive randomly in each stream, with new packets making the previous ones obsolete. In this case, we consider the version age of information (VAoI) at a user, defined as the difference in the version index of the latest available packet at the BS and that at the user, as a metric of freshness of information. Our objective is to minimize a weighted sum of average VAoI across users subject to an average power constraint at the BS by optimally scheduling the update packets from various streams for transmission and transmitting them with sufficient powers to guarantee their successful delivery. We consider the class of channel-only stationary randomized policies (CO-SRP), which rely solely on channel power gains for transmission decisions. We solve the resulting non-convex problem optimally and show that the VAoI achieved under the optimal CO-SRP is within twice the optimal achievable VAoI. We also obtained a Constrained Markov Decision Process (CMDP)-based solution and its structural properties. Numerical simulations show a close performance between the optimal CO-SRP and CMDP-based solutions. Additionally, a time division multiple access (TDMA) scheme, which allows transmission to at most one user at a time, matches NOMA's performance under tight average power constraints. However, NOMA outperforms TDMA as the constraint is relaxed.

==> References/fig1.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={$\beta$},
xmin=-0.01895, xmax=0.41995,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Objective Function},
ymin=-243.727689793909, ymax=5288.35843005382,
ytick style={color=black}
]
\addplot[color=red, dashed,thick, mark=square, mark options={solid, red}, mark size = 2pt]
table {%
0.001 154.242348906481
0.005 149.385255045914
0.01 93.9447384690876
0.05 11.8042169975681
0.1 7.73077019916978
0.15 32.6510687390864
0.2 69.5995013995039
0.3 68.7538913534642
0.4 70.5842962315175
};
\addlegendentry{MDP}
\addplot[color=blue, dashed,thick, mark=square, mark options={solid, blue}, mark size = 2pt]
table {%
0.001 5036.89997006074
0.005 1334.53464944554
0.01 807.830396669139
0.05 301.433614700474
0.1 281.273735608493
0.15 240.143727121818
0.2 197.807541725635
0.3 175.454141517188
0.4 176.247669712004
};
\addlegendentry{Stationary Randomized Policy}
\end{axis}

\end{tikzpicture}



 


==> References/fig2.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={VAOI of Stream 1},
xmin=-0.2211205, xmax=4.6435305,
xtick style={color=black},
y grid style={darkgray176},
ylabel={VAOI of Stream 2},
ymin=-0.1977065, ymax=4.1518365,
ytick style={color=black}
]
\addplot [semithick, steelblue31119180]
table {%
0 1.38301
0.55199 1.206975
1.1107675 1.0313925
1.65839625 0.86433125
2.235135 0.69229
2.7526375 0.51604125
3.3254925 0.3457175
3.88983875 0.1720925
4.42241 0
};
\addlegendentry{MDP}
\addplot [semithick, darkorange25512714]
table {%
0 3.95413
0.118115 3.32878875
0.24055 2.869605
0.36795375 2.42663125
1.66674 2.28262
2.1263375 2.54654625
2.67132 3.53529
3.24711625 1.83255375
3.71535 0
};
\addlegendentry{SRP}
\end{axis}

\end{tikzpicture}


==> References/fig3-1.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\end{tikzpicture}


==> References/fig3.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\end{tikzpicture}


==> References/tab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Variation of the long-term average expected VAoIs of User $1$ and User $2$ and the transmit powers allocated to the Stream $1$ and Stream $2$ at the BS for superposition coding.}
\centering
	\begin{tabular}{c|cc|cc}
	\hline
	\multicolumn{1}{c|}{\multirow{2}{*}{$\beta$}} & \multicolumn{2}{c|}{Long-Term Average VAoI}              & \multicolumn{2}{c}{Long-Term Average Power}                                            \\ \cline{2-5} 
	\multicolumn{1}{c|}{}                      & \multicolumn{1}{c|}{User $1$}  & \multicolumn{1}{c|}{User $2$} & \multicolumn{1}{c|}{Stream $1$}         & \multicolumn{1}{c}{Stream $2$} \\ \hline
	%1.00E-05                                   & \multicolumn{1}{l|}{0.3493925} &                               & \multicolumn{1}{l|}{2272.71094940026} &                              \\ \hline
	%5.00E-05                                   & \multicolumn{1}{l|}{0.3491125} &                               & \multicolumn{1}{l|}{2272.34590245872} &                              \\ \hline
	%0.0001                                     & \multicolumn{1}{l|}{0.3504375} &                               & \multicolumn{1}{l|}{2325.54245073357} &                              \\ \hline
	0.0005                                     & \multicolumn{1}{l|}{0.55} & 0.87                     & \multicolumn{1}{l|}{268.21} & 4125.14             \\ \hline
	0.001                                      & \multicolumn{1}{l|}{0.58} & 1.21                      & \multicolumn{1}{l|}{149.92} & 1514.14             \\ \hline
	0.005                                      & \multicolumn{1}{l|}{0.60}  & 0.93                      & \multicolumn{1}{l|}{145.76}  & 1514.33             \\ \hline
	0.01                                       & \multicolumn{1}{l|}{0.73}   & 0.89                       & \multicolumn{1}{l|}{88.59} & 1257.53             \\ \hline
	0.05                                       & \multicolumn{1}{l|}{1.60} & 1.58                     & \multicolumn{1}{l|}{10.41}  & 262.36             \\ \hline
	0.1                                        & \multicolumn{1}{l|}{2.74} & 2.86                     & \multicolumn{1}{l|}{2.289} & 197.93             \\ \hline
	%0.5                                        & \multicolumn{1}{l|}{4.6196575} & 6.2926575                     & \multicolumn{1}{l|}{54.3142549020765} & 164.434081724963             \\ \hline
	%1                                          & \multicolumn{1}{l|}{4.6394375} & 6.389865                      & \multicolumn{1}{l|}{52.6142862891098} & 163.659292648332             \\ \hline
	\end{tabular}
 \label{tab:VAoI-Power}

\end{table}
